Gamma-Ray Burst Observations at High Energy with the Fermi Large Area Telescope

The Fermi Gamma-ray Space Telescope with its main instrument onboard, the Large Area Telescope (LAT), opened a new era in high-energy astrophysics and in particular for the study of Gamma-Ray Bursts (GRBs), which are short flashes of -rays associated with the brightest and most distant events ever observed in our universe after the Big Bang. My thesis work focused primarily on the observations of this phenomenon with the LAT (20 MeV - 300 GeV) and the Gamma-ray Burst Monitor (10 keV - 40 MeV) onboard the Fermi satellite. After describing the procedure used for detection and analysis of LAT GRBs, I will provide an overview of the temporal and spectral features observed during the prompt emission of these events after one year and a half of operation for Fermi. GRBs can also be used as a tool to probe interesting physics. My focus will be on the detection of very high energy photons (typically above 10 GeV) associated with LAT GRBs and which were used to set significant constraints both on a possible violation of Lorentz invariance - which postulates that all observers measure exactly the same speed of light in vacuum, independently of photon energy - and on the Optical-Ultraviolet extragalactic background light in the Universe.

==> Chapters/test.tex <==
\chapter{\label{chap:test}Test}

skfjsldkf

==> Chapters/tmp/Intro_GRB_expectation_paper.tex <==
\chapter{GRB Introduction}

\section{general GRB introduction}

\section{GRBs at high-energy in the pre-Fermi era}

\subsection{Previous Observations}\label{sec:Previous_Observations}

The detectors of the {\it Compton Gamma-Ray Observatory (CGRO)}
provided time-resolved spectra for a statistically well-defined
burst population.  These observations are the foundation of our
expectations for $Fermi$'s discoveries, which have guided the
development of analysis tools before launch.

The Burst And Transient Source Experiment (BATSE) on {\it CGRO}
observed a large sample of bursts in the $\sim$25--2000~keV band
with well-understood population statistics \citep{Paciesas:99}.
Spectroscopy by the BATSE detectors found that the emission in this
energy band could be described by the empirical four parameter
``Band'' function \citep{Band:93}
%
\begin{equation}
\label{eqn:BandF2}
%
N_{\rm Band}(E | N_0,E_p,\alpha,\beta) = N_0 \left\{
\begin{array}{l l}
   E^{\alpha} \exp[-E(2+\alpha)/E_p], &  E \le {{\alpha-\beta}\over {2+\alpha}} E_p \\
\\
   E^\beta \left[ {{\alpha-\beta}\over {2+\alpha}} E_p\right]^{(\alpha-\beta)}
   \exp[\beta-\alpha] , & E > {{\alpha-\beta}\over {2+\alpha}} E_p,
\end{array}
\right.
\end{equation}
%
where $\alpha$ and $\beta$ are the low and high energy
photon indices, respectively, and $E_p$ is the `peak
energy' which corresponds to the maximum of $E^2 N(E)
\propto \nu f_\nu$ for the low energy component. Typically
$\alpha \sim -0.5$ to $-1$ and $\beta$ is less than $-2$
\citep{Band:93,Preece:00,Kaneko:06}; the total energy would
be infinite if $\beta \geq -2$ unless the spectrum has a
high energy cutoff. The observations of 37 bursts by the
Compton Telescope (COMPTEL) on {\it CGRO} (0.75--30~MeV)
are consistent with the BATSE observations of this spectral
component \citep{Hoover:05}. Because of the relatively poor
spectral resolution of the BATSE detectors
\citep{Briggs:99}, this functional form usually is a good
description of spectra accumulated over both short time
periods and entire bursts, even though bursts show strong
spectral evolution \citep{Ford:95}.  It is this
10--1000~keV `prompt' component that is well-characterized
and therefore provides a basis for quantitative
predictions. A detailed duration-integrated spectral
analysis (in ~30 keV-200 MeV) of the prompt emission for 15
bright BATSE GRB performed by \citet{Kaneko:08} confirmed
that only in few case there's a significant high-energy
excess with respect to low energy spectral extrapolations.

% more on this?

The burst observations by the Energetic Gamma-Ray
Experiment Telescope (EGRET) on {\it CGRO} (20~MeV to
30~GeV) provide the best prediction of the LAT
observations.  EGRET observed different types of high
energy burst phenomena. Four bursts had simultaneous
emission in both the EGRET and BATSE energy bands,
suggesting that the spectrum observed by BATSE extrapolates
to the EGRET energy band \citep{Dingus:03}.  However, the
correlation with the prompt phase pulses was hampered by
the severe EGRET spark chamber dead time
($\sim$100~ms/event) that was comparable or longer than the
pulse timescales.  The EGRET observations of these bursts
suggest that the $\sim$1~GeV emission often lasts longer
than the lower energy emission, and thus results in part
from a different physical origin. 
A similar behaviour is present also in GRB 080514B detected by AGILE\citep{Giuliani:08}.

Whether high energy emission is present in both long and
short bursts is unknown. The four bursts with high energy
emission detected by EGRET were all long bursts, although
GRB 930131 is an interesting case. It was detected by BATSE
\citep{Kouveliotou:94} with duration of $T_{90}$=14~s
\footnote{$T_{90}$ is the time over which 90\% of the
emission occurs in a specific energy band.} and found to
have high-energy ($>$30~MeV) photons accompanying the
prompt phase and possibly extending beyond
\citep{Sommer:94}.  The BATSE lightcurve is dominated by a
hard initial emission lasting ~1 sec and followed by a smooth
extended emission. This burst may, therefore, have been one
of those long bursts possibly associated with a merger and
not a collapsar origin, commonly understood as the most
probable origin for short and long burst
respectively\citep{Zhang:07}. Several events have now been
identified that could fit into this category
\citep{Norris:06} and their origin is still uncertain. LAT
will make an important contribution in determining the
nature of the high energy emission from similar events and
a larger sample of bursts with detected high energy
emission will determine whether the absence of high energy
emission differentiates short from long bursts.

%Sixteen photons $>$30~MeV were
%detected from GRB~930131 during, and possibly after, the
%prompt phase \citep{Sommer:94}. While the BATSE duration of
%$T_{90}$=14~s \citep{Kouveliotou:94}\footnote{$T_{90}$ is
%the time over which 90\% of the emission occurs} would
%appear to categorize this as a long burst, GRB~930131 may
%have been a short GRB with extended emission
%\citep{Norris:06} since the BATSE lightcurve is a hard
%initial spike lasting $\sim$1~s followed by softer extended
%emission. Thus it is uncertain whether this GRB was a
%member of the long or short burst populations, and no other
%EGRET-detected burst was short.

A high energy temporally resolved spectral component in
addition to the Band function is clearly present in GRB
941017 \citep{Gonzalez:03}; this component is harder than
the low energy prompt component, and continues after the
low energy component fades into the background.  The time
integrated spectra of both GRB~941017 and GRB~980923 show
this additional spectral component \citep{Kaneko:08}.

Finally, the $>$1~GeV emission lingered for 90~minutes
after the prompt low energy emission for GRB~940217,
including an 18~GeV photon 1.5 hours after the burst
trigger \citep{Hurley:94}.  Whether this emission is
physically associated with the lower energy afterglows is
unknown.

These three empirical types of high energy emission---an
extrapolation of the low energy spectra; an additional spectral
component during the low energy prompt emission; and an
afterglow---guide us in evaluating $Fermi$'s burst observation
capabilities.

Because the prompt low energy component was characterized
quantitatively by the BATSE observations while the EGRET
observations merely demonstrated that different components were
present, our simulations are based primarily on extrapolations of
the prompt low energy component from the BATSE band to the
$>$100~MeV band.  We recognize that the LAT will probably detect
additional spectral and temporal components, or spectral cutoffs,
that are not treated in this extrapolation.

During the first few months of the $Fermi$ mission, LAT detected already emission from three GRBs: 080825C \citep{Bouvier:08}, 080916C \citep{Tajima:08} and 081024B \citep{Omodei:08}. The rich phenomenology of high energy emission is confirmed in these three events, where spectral measurements over various order of magnitude were possible together with the detection of extended emission and spectral lags. 
In particular, the GRB 080916C was bright enough to afford unprecedented broad-band spectral coverage in four distinct time intervals \citep{Abdo:09}, thereby offering new insights into the character of energetic bursts. 


\subsection{Theoretical Expectations}\label{sec:Theory}

In the current standard scenario, the burst emission arises
in a highly relativistic, unsteady outflow.  Several
different progenitor types could create this outflow, but
the initial high optical depth within the outflow obscures
the progenitor type. As this outflow gradually becomes
optically thin, dissipation processes within the outflow,
as well as interactions with the surrounding medium, cause
particles to be accelerated to high energies and loose some
of their energy into radiation. Magnetic fields at the
emission site can be strong and may be caused by a
frozen-in component carried out by the outflow from the
progenitor, or may be built up by turbulence or
collisionless shocks. The emitted spectral distribution
then depends on the details of the radiation mechanism,
particle acceleration, and the dynamics of the explosion
itself.

`Internal shocks' result when a faster region catches up with a
slower region within the outflow. `External shocks' occur
at the interface between the outflow and the ambient
medium, and include a long-lived forward shock that is
driven into the external medium and a short-lived reverse
shock that decelerates the outflow.  Thus the simple model
of a one-dimensional relativistic outflow leads to a
multiplicity of shock fronts, and many possible interacting
emission regions.

As a result of the limited energy ranges of past and current
experiments, most theories have not been clearly and unambiguously
tested. $Fermi$'s GBM and LAT will provide an energy range broad
enough to distinguish between different origins of the emission; in
particular the unprecedented high-energy spectral coverage will
constrain the total energy budget and radiative efficiency, as
potentially most of the energy may be radiated in the LAT range. The
relations between the high and low energy spectral components can
probe both the emission mechanism and the physical conditions in the
emission region. The shape of the high energy spectral energy
distribution will be crucial to discriminate between hadronic
cascades and leptonic emission.  The spectral breaks at high energy
will constrain the Lorentz factor of the emitting region. Previously
undetected emission components might be present in the light curves
such as thermal emission. Finally, temporal analysis of the high
energy delayed component will clarify the nature of the flares seen
in the X-ray afterglows.

\subsubsection{Leptonic vs. Hadronic Emission
Models}\label{sec:Leptonic_Hadronic}

It is very probable that particles are accelerated to very
high energies close to the emission site in GRBs. This
could either be in shock fronts, where the Fermi mechanism
or other plasma instabilities can act, or in magnetic
reconnection sites. Two major classes of
models---synchrotron and inverse Compton emission by
relativistic electrons and protons, and hadronic
cascades---have been proposed for the conversion of
particle energy into observed photon radiation.

In the leptonic models, synchrotron emission by relativistic
electrons can explain the 10~keV--1~MeV spectrum in $\sim$2/3 of
bursts (e.g., see \citealt{Preece:98}), and inverse Compton (IC)
scattering of low energy seed photons generally results in GeV band
emission.  These processes could operate in both internal and
external shock regions (see, e.g., \citealt{Zhang:01}), with the
relativistic electrons in one region scattering the `soft' photons
from another region
\citep{Fragile:04,Fan:05,Meszaros:94,Waxman:97,Panaitescu:98}.
Correlated high and low energy emission is expected if the same
electrons radiate synchrotron photons and IC scatter soft photons.
In Synchrotron Self-Compton (SSC) models the electrons' synchrotron
photons are the soft photons and thus the high and low energy
components should have correlated variability
\citep{Guetta:03,Galli:08}. However, SSC models tend to generate
a broad $\nu F_{\nu}$ peak in the MeV band, and for bursts observed
by {\it CGRO} this breadth has difficulty accommodating the observed
spectra \citep{Baring:04}. $Fermi$, with its broad spectral coverage
enabled by the GBM and the LAT, is ideally suited for probing this
issue further.

Alternatively, photospheric thermal emission might dominate
the soft keV--MeV range during the early part of the prompt
phase \citep{Rees:05,Ryde:04,Ryde:05}.  Such a component is
expected when the outflow becomes optically thin, and would
explain low energy spectra that are too hard for
conventional synchrotron models
\citep{Crider:97,Preece:98,Preece:02}. An additional power
law component might underlie this thermal component and
extend to high energy; this component might be synchrotron
emission or IC scattering of the thermal photons by
relativistic electrons.  Fits of the sum of thermal and
power law models to BATSE spectra have been successful
\citep{Ryde:04,Ryde:05}, but joint fits of spectra from the
two types of GBM detectors and the LAT should resolve
whether a thermal component is present
\citep{Battelino:07a, Battelino:07b}.

In hadronic models relativistic protons scatter inelastically off
the $\sim$100~keV burst photons ($p\gamma$ interactions) producing
(among other possible products) high-energy, neutral pions ($\pi^0$)
that decay, resulting in gamma rays and electrons that then radiate
additional gamma rays. Similarly, if neutrons in the outflow
decouple from protons, inelastic collisions between neutrons and
protons can produce pions and subsequent high energy emission
\citep{Derishev:00,Bahcall:00}. High energy neutrinos that may be
observable are also emitted in these interactions
\citep{Waxman:97a}.  Many variants of hadronic cascade models have
been proposed: high energy emission from proton-neutron inelastic
collisions early in the evolution of the fireball
\citep{Bahcall:00}; proton-synchrotron and photo-meson cascade
emission in internal shocks (e.g.,
\citealt{Totani:98,Zhang:01,Fragile:04,Gupta:07}); and proton
synchrotron emission in external shocks \citep{Bottcher:98}.  A
hadronic model has been invoked to explain the additional spectral
component observed in GRB~941017 \citep{DermerAtoyan:04}. The
emission in these models is predicted to peak in the MeV to GeV band
\citep{Bottcher:98,Gupta:07}, and thus would produce a clear signal
in the LAT's energy band. However, photon-meson interactions would
result from a radiatively inefficient fireball \citep{Gupta:07},
which is in contrast with the high radiative efficiency that is
suggested by {\it Swift} observations \citep{Nousek:06,Granot:06}.
Thus, the hadronic mechanisms for gamma-ray production
are many, but the $Fermi$ measurements of the temporal evolution of
the highest energy photons will provide strong constraints on these
models, and moreover discern the existence or otherwise of distinct GeV-band components.

\subsubsection{High-Energy Absorption}\label{sec:HE_abs}

At high energies the outflow itself can become optically
thick to photon-photon pair production, causing a break in
the spectrum. Signatures of internal absorption will
constrain the bulk Lorentz factor and adiabatic/radiative
behavior of the GRB blast wave as a function of time
\citep{Baring:97,Lithwick:01,Guetta:03,Baring:06,Granot:08}.
Since the outflow might not be steady and may evolve during
a burst, the breaks should be time-variable, a distinctive
property of internal attenuation.  Moreover, if the
attenuated photons and their hard X-ray/soft gamma-ray
target photons originate from proximate regions in the
bursts, the turnovers will approximate broken power-laws. Interestingly, 
the LAT has already provided palpable new
advances in terms of constraining bulk motion in bursts.  For
GRB 080916C, the absence of observable attenuation turnovers up
to around 13 GeV suggests that the bulk Lorentz factor may be
well in excess of 500-800 \citep{Abdo:09}.

Spectral cutoffs produced by internal absorption must be
distinguished observationally from cutoffs caused by interactions
with the extragalactic background. The optical depth of the Universe
to high-energy gamma rays resulting from pair production on infrared
and optical diffuse extragalactic background radiation can be
considerable, thereby preventing the radiation from reaching us.
These intervening background fields necessarily generate
quasi-exponential turnovers familiar to TeV blazar studies, which
may well be discernible from those resulting from internal
absorption. Furthermore, their turnover energies should not vary
with time throughout the burst, another distinction between the two
origins for pair attenuation. In addition, the turnover energy for
external absorption is expected above a few 10's of GeV while for
internal absorption it may be as low as $\leq 1\;$GeV
\citep{Granot:08}. Although the external absorption may complicate
the study of internal absorption, studies of the cutoff as a
function of redshift can measure the universe's optical energy
emission out to the Population~III epoch (with redshift $> 7$)
\citep{deJager:02,Coppi:97,Kashlinsky:05,BrommLoeb:06}.

\subsubsection{Delayed GeV Emission}

The observations of GRB~940217 \citep{Hurley:94}
demonstrated the existence of GeV-band emission long after
the $\sim$100~keV `prompt' phase in at least some bursts.
With the multiplicity of shock fronts and with synchrotron
and IC components emitted at each front, many models for
this lingering high energy emission are possible. In
combination with the prompt emission observations and
afterglow observations by {\it Swift} and ground-based
telescopes, the LAT observations may detect spectral and
temporal signatures to distinguish between the different
models.

These models include:  Synchrotron Self-Compton (SSC)
emission in late internal shocks (LIS)
\citep{Zhang:02,Wang:06,Fan:08,Galli:08}; external IC (EIC)
scattering of LIS photons by the forward shock electrons
that radiate the afterglow \citep{Wang:06}; IC emission in
the external reverse shock (RS)
\citep{Wang:01,Granot:03,Kobayashi:07}; and SSC emission in
forward external shocks
\citep{MeszarosRees:94,Dermer:00b,Zhang:01,Dermer:07,Galli:07}.

A high energy IC component may be delayed and have broader
time structures relative to lower energy components because
the scattering may occur in a different region from where
the soft photons are emitted \citep{Wang:06}.  The
correlation of GeV emission with X-ray afterglow flares
observed by {\it Swift} would be a diagnostic for different
models \citep{Wang:06,Galli:07,Galli:08}.

\subsection{Timing Analysis}

The LAT's low deadtime and large effective area will permit
a detailed study of the high energy GRB light curve, which
was impossible with the EGRET data as a result of the large
deadtime that was comparable to typical widths of the peaks
in the lightcurve. These measures are clearly important for
determining the emission region size and the Lorentz factor
in the emitting fireball.

The lightcurves of GRBs are frequently complex and diverse.
Individual pulses display a hard-to-soft evolution, with
$E_p$ decreasing exponentially with the burst flux. One
method of classifying bursts is to examine the spectral
lag, which relates to the delay in the arrival of high
energy and low energy photons
\citep[e.g.,][]{Norris:00,Foley:08}. A positive lag value
indicates hard-to-soft evolution
\citep{Kocevski:03,Hafizi:07}, i.e., high energy emission
arrives earlier than low energy emission. This lag is a
direct consequence of the spectral evolution of the burst
as $E_p$ decays with time. The distributions of spectral
lags of short and long GRBs are noticeably different, with
the lags of short GRBs concentrated in the range $\pm$
30\,ms \citep[e.g.,][]{Norris:06,Yi:06}, while long GRBs
have lags covering a wide range with a typical value of
100\,ms \citep[e.g.,][]{Hakkila:07}. \citet{Stamatikos:08}
study the spectral lags in the {\it Swift} data.

An anti-correlation has been discovered between the lag and the peak
luminosity of the GRB at energies $\sim$ 100\,keV \citep{Norris:00},
using six BATSE bursts with definitive redshift. Brighter long GRBs
tend to have a high peak luminosity and short lag, while weaker GRBs
tend to have lower luminosities and longer lags. This
``lag--luminosity relation'' has been confirmed by using a number of
\textit{Swift} GRBs with known redshift \citep[e.g., GRB~060218,
with a lag greater than 100~s, ][]{Liang:06}. $Fermi$ will be able to
determine if this relation extends to MeV-GeV energies.

A subpopulation of local, faint, long lag GRBs has been proposed by
\citet{Norris:02} from a study of BATSE bursts, which implies that
events with low peak fluxes ($F_{P} (50-300\hbox{ keV}) \sim
0.25$\,ph\,cm$^{-2}$\,s$^{-1}$) should be predominantly long lag
GRBs. \citet{Norris:02} successfully tested a prediction that these
long lag events are relatively nearby and show some spatial
anisotropy, and found a concentration towards the local
supergalactic plane. This has been confirmed with the GRBs observed
by INTEGRAL \citep{Foley:08}  where it was found that $>$\,90\% of
the weak GRBs with a lag $>0.75$\,s were concentrated in the
supergalactic plane. $Fermi$ measures of long lag GRBs will confirm
this hypothesis.  An underluminous abundant population is inferred
from observations of nearby bursts associated with supernovae
\citep{Soderberg:06}.

Moreover, some Quantum Gravity (QG) theories predict an
energy dependent speed-of-light (see e.g.,
\citealt{Mattingly:05}), which is often parameterized as
%
\begin{equation}
v = c\left(1-\left(E(z)/E_{qg}\right)\right)
\end{equation}
%
where $E(z)$ is the photon energy at a given redshift, $E(z)=
E_{obs}(1+z)$, and $E_{qg}$ is the QG scale, which may be of order
$\sim 10^{19}$~GeV.  This energy-dependence can be measured from the
difference in the arrival times of different-energy photons that
were emitted at the same time; measurements thus far give $E_{qg}$
greater than a few times $10^{17}$~GeV.  Such photons might be
emitted in sharp burst pulses \citep{Amelino-Camelia:98};
measurements have been attempted \citep{Schaefer:99,Boggs:04}.  With
the energy difference between the GBM's low energy end and the LAT's
high energy end, the good event timing by both the GBM and the LAT,
and the LAT's sensitivity to high energy photons, the $Fermi$ mission
will place interesting limits on $E_{qg}$.


==> Chapters/tmp/Introduction_GRB.tex <==
\chapter{\label{chap:GRB}Gamma-Ray Bursts}

\section{Introduction}

Gamma-Ray Bursts (GRBs) are the brightest explosions ever observed in our universe. 
They are brief and bright transient emissions of $keV/MeV$ radiation, 
occurring with a rate of a few per day uniformly in the sky. Even
though they are at cosmological distances (up to Gigaparsecs or $\sim10^{28}\,cm$), 
they outshine all other sources in the gamma-ray sky during their short period of emission. The energy output of a single GRB in keV/MeV gamma rays is comparable to the emission of all the stars of a galaxy in all the electromagnetic spectrum, during more than a 100 years.

The initial (prompt) emission of GRBs is brief (milliseconds to minutes), highly variable
(in time scales of $ms$ to tens of seconds), non-thermal, and observed
mostly in the keV/MeV energy range. The emission is believed to be produced
by electrons accelerated during collisionless shocks inside highly collimated relativistic
jets. For the majority of GRBs, the prompt emission is followed by
a smoothly decaying and long-lasting ``afterglow, '' observed in
longer wavelengths (from X-rays to optical), and believed to be produced by the deceleration
of the relativistic jet in the surrounding interstellar or circumburst
medium. GRBs of long durations (typically $\gtrsim\,2s$) are likely to be produced by the collapse of the cores of massive spinning stars. The progenitor of shorter duration GRBs ($\lesssim\,2s$) is less certain although mergers of compact binaries (neutron star-neutron star or neutron star-black hole) seem good candidate.

High-redshift GRBs are 100 to 1000 times brighter than high-redshift
QSOs\footnote{QSO: Quasi-Stellar Object, an extremely powerful and distant active
galactic nucleus.}, and also expected to occur out to at least redshifts $z\simeq 10$ and possibly up to $z\simeq 15-20$, 
while QSOs occur only out to redshift $z\sim7$ \citep{Lamb01}. Therefore, GRBs are unique tools for probing
the very distant (or very young) universe as early in time as the
epoch of reionization (Fig. \ref{fig:GRB_Times}). GRBs can be used
to learn about the evolution history of the universe (star formation history, 
metallicity at different redshifts), its large-scale structure, and
the properties of the earliest generations of stars. %
\begin{figure}[ht]
\begin{centering}
\includegraphics[width=0.8\columnwidth]{Plots/GRBs/Lamb}
\par\end{centering}

\caption{\label{fig:GRB_Times}Cosmological context of GRBs. Contrary to quasi-stellar objects, 
gamma-ray bursts can help us probe the properties of the universe as early in time as
the epoch of reionization. Source: \cite{GRB_Lamb_Reichart_2001}}

\end{figure}
The afterglow of GRBs passes through multiple regions filled with
gas or radiation fields before it reaches the earth (Fig. \ref{fig:GRB_Stuff}). 
Spectroscopic studies on the absorption features imprinted on the
GRB afterglow at each of these regions provide unique information
regarding the regions' composition and density \cite{GRB_Prochaska_et_al2007}. 
GRBs are also believed to be intense sources of neutrinos, cosmic
rays (up to ultra-high energies $10^{20}\,eV$), and gravitational waves. Observations
of these emissions can answer questions in astrophysics, 
particle physics, and general relativity. 

The diverse and intriguing properties of GRBs make them the focus
of intense scientific research and debate (Fig. \ref{fig:GRB_Papers}), 
and the observational target of multiple instruments (Fig. \ref{fig:GRB_Experiments}). 
Despite the fact that we have known about GRBs for over thirty five years, 
and that more than eight thousand refereed papers have been written about them, 
they still continue to spark scientific interest. The commissioning
of new detectors sensitive to GRB's keV to GeV gamma-ray emission, 
such as the GBM and the LAT aboard GLAST \cite{URL_GLAST}; to their GeV/TeV
emission, such as HAWC \cite{URL_HAWC}; sensitive to their neutrino emission,
such as IceCube \cite{URL_ICECUBE}; and sensitive to their gravitational-wave emission, such as LISA \cite{URL_LISA},
will surely renew interest and raise new questions. %
\begin{figure}[ht]
\includegraphics[width=1\columnwidth]{Plots/GRBs/Stuff}

\caption{\label{fig:GRB_Stuff}Schematic of the various environments intersected
by a GRB line of sight. The GRB emission passes through the circumstellar
medium (CSM) around the GRB progenitor; the star-forming region surrounding
the GRB (HII Region, $H_{2}$ Cloud); the ambient interstellar medium (ISM)
of the host galaxy; the baryonic halo of the galaxy (Halo gas); 
and the intergalactic medium (IGM) between the earth and the GRB.
The absorption features imprinted on the GRB signal as it passes through
these regions can reveal information about their density and composition. Source:
\cite{GRB_Prochaska_et_al2007}}
\end{figure}
%

\begin{figure}[ht]
\begin{centering}
\includegraphics[width=0.8\columnwidth]{Plots/GRBs/dPaper}
\par\end{centering}

\caption{\label{fig:GRB_Papers}Number of GRB-related refereed publications
per year. Source: \cite{URL_hurley}}

\end{figure}


\begin{figure}[ht]
\includegraphics[angle=270, width=1\columnwidth]{Plots/GRBs/experimentstable}
\caption{\label{fig:GRB_Experiments}List of experiments sensitive to GRBs and approximate
numbers of detected GRBs (as of early May 2008). Source: \cite{URL_JeanZand}}
\end{figure}


This chapter will give an overview of our current knowledge regarding GRBs.
A historical overview of GRB observations will be given in section
\ref{sec:GRBs_History}, and the currently accepted
model for the progenitor and mechanism of GRBs will be presented in
section \ref{sec:GRB_Hosts}. 


\section{\textmd{\label{sec:GRBs_History}}History of GRB Observations}


\subsection{The first years (1967-1991)}

Well before GRBs became publicly known, Colgate hypothesized their existence,
associating them with the ejection of
relativistic shocks from supernovae \cite{GRB_Colgate_1968}. GRBs
were accidentally discovered in 1967 by the US Vela satellites, 
operated by Los Alamos National Laboratory \cite{GRB_Dickinson_Tamarkin_1965}, 
whose purpose was to monitor from space, for violations of the nuclear-test ban
treaty. The Vela satellites carried omnidirectional detectors
sensitive to the gamma-ray pulses emitted by nuclear-weapon explosions. 
However, their detectors were also sensitive to the gamma-ray emission from GRBs. 
Soon after they were launched, they started detecting bursts of gamma rays
that were, fortunately, identified as coming from space. 
The detection of the first GRBs was immediately classified and was
not made public until seven years later \cite{GRB_Discovery}, when
sixteen GRB detections were reported in the $0.2-1.5\,MeV$ energy range. After
the Vela satellites, a number of instruments were dedicated to detecting
GRBs (Fig. \ref{fig:GRB_Experiments}). However, the number
of bursts detected was small and the angular resolution poor. 


\subsection{BATSE (1991-2000)}

A breakthrough in our understanding of GRBs happened with the numerous
GRB detections from the Burst And Transient Source Explorer (BATSE) \cite{URL_BATSE}
, which flew, with other instruments, on board the Compton Gamma-Ray Observatory
 (CGRO) \cite{URL_CGRO}. BATSE operated from 1991 to 2000. 
It was sensitive to the $15\,keV-2\,MeV$ energy
range, had a wide field of view ($4\pi\,sr$ minus 30\% because of
earth obscuration), and a moderate angular resolution ($\sim4^{o}$). 
It detected 2704 GRBs \cite{GRB_Paciesas_et_al1999}, a significantly
larger number than the total number of GRBs in the pre-existing catalog
(few hundreds). In combination with the Energetic Gamma-Ray Experiment
Telescope (EGRET) \cite{URL_EGRET}, a gamma-ray detector also aboard the CGRO, GRB observations
in the extended energy range $15\,keV-30\,GeV$ were made. 

Before BATSE, the distance scale of GRBs was unknown. The
scientific community was divided among multiple theories predicting
distance scales ranging from our own galaxy to the edges of the known
universe. Even though GRBs were observed uniformly, it was
believed that they come from galactic neutron stars. It was believed that
the reason we saw a uniform-in-space distribution instead the pancake shape
of our galaxy was that the pre-BATSE instruments were not sensitive enough
to probe deep enough and see the galactic structure 

BATSE was sensitive enough to detect GRBs originating from distances 
larger than the size of our galaxy. 
Its discovery that GRBs are isotropically distributed
(Fig. \ref{fig:GRB_Locations}) narrowed down the possibilities
and suggested that GRBs are most probably located at cosmological distances
further away than our local group of galaxies. Otherwise, the GRB
spatial distribution would be correlated with the local distribution
of mass (our galaxy, the LMC, M31, globular clusters, the Virgo cluster, 
etc.) and would not be isotropic. However, the distance-scale
problem was not completely resolved, because an extended halo around our
galaxy could still generate a uniform distribution similar to the
one observed. %

\begin{figure}[ht]
\includegraphics[width=1\columnwidth]{Plots/GRBs/batselocations}
\caption{\label{fig:GRB_Locations}Locations of all the 2704 GRBs detected
by BATSE in galactic coordinates. The plane of our galaxy is along
the horizontal line at the middle of the figure. The isotropic distribution
of GRBs in space implied that GRBs are most likely cosmological
sources. Source: \cite{URL_BATSE_Locations}}
\end{figure}

Some GRB properties emerged from the extensive dataset of BATSE-detected GRBs. 
The light curves of GRBs showed great morphological diversity,
ranging from smooth, fast rise, and quasi-exponential decays, 
to curves with many peaks and with a high variability, ranging
from timescales of milliseconds to many minutes (Fig. \ref{fig:GRB_TimeCurves}). 
%
\begin{figure}[ht]
\includegraphics[width=1\columnwidth]{Plots/GRBs/grb_profiles}
\caption{\label{fig:GRB_TimeCurves}Light curves of some of the GRBs detected
by BATSE. The light curves of GRBs show great variability and diversity. 
Source: J. T. Bonnell (NASA/GSFC)}
\end{figure}


The duration of GRBs is usually described by the $T_{90}$ parameter, 
which is equal to the time over which the burst emits from 5\% to
95\% of its measured counts. The $T_{90}$ distribution of GRBs
(Fig. \ref{fig:GRB_T90}) spans a long range of durations and
has a bimodal shape. Based on that, GRBs were divided into two categories:
``short bursts'' having $T_{90}\lesssim2\,s$, and ``long bursts''
having $T_{90}\gtrsim2\,s$. Short bursts constituted $\sim30\%$
of the BATSE sample. The spectral properties of short and long GRBs were different. 
BATSE measured the fluence of a burst in different channels, each
one corresponding to a different energy range. The ``Hardness Ratio,''
defined as the ratio of the fluence in channel 3 ($100-300\,keV$)
over the fluence in channel 2 ($50-100\,keV$), was a measure of the spectral
hardness of a burst. Short bursts were found to have on average higher hardness 
ratios than long bursts, as shown on figure \ref{fig:GRB_HardnessRatio}. 
The existence of two distinct populations of bursts implied the existence of two
kinds of progenitors and inner engines. 


\begin{figure}[ht]
\begin{centering}
\includegraphics[width=0.8\columnwidth]{Plots/GRBs/t90}
\par\end{centering}

\caption{\label{fig:GRB_T90}Duration ($T_{90}$) distribution of 
the GRBs detected by BATSE. Two populations of bursts, separated at $T_{90}\simeq2\,s$, 
can be seen. Source: \cite{URL_BATSE_Durations}}
\end{figure}

\begin{figure}[ht]
\begin{centering}
\includegraphics[width=0.8\columnwidth]{Plots/GRBs/HardnessRatio}
\par\end{centering}

\caption{\label{fig:GRB_HardnessRatio}Hardness ratio versus duration $(T_{90})$
for BATSE GRBs. Short bursts ($T_{90}\lesssim2\,s$) have higher hardness 
ratios than long bursts ($T_{90}\gtrsim2\,s$), supporting the 
hypothesis that short and long bursts constitute two separate populations, 
probably originating from different progenitors. Source : \cite{GRB_Hjorth_et_al2005} }

\end{figure}

The measured spectra were not thermal, and evolved with time from hard to soft. 
The time-averaged spectrum followed an \textit{ad hoc} function, 
called the ``Band function'' $S(E)$ \cite{GRB_Band_et_al_1993}, 
given by:

\begin{equation}
S(E)=A\times\begin{cases}
\left(\frac{E}{100keV}\right)^{a}e^{-\frac{E}{E_{0}}} & E\le(a-\beta)E_{0}\\
\left(\frac{(a-\beta)E_{0}}{100keV}\right)^{\alpha-\beta}\left(\frac{E}{100keV}\right)^{\beta}e^{\beta-\alpha} & E\ge(a-\beta)E_{0},\end{cases}\label{eq:GRB_BandFunction}\end{equation}
where $a$ and $\beta$ are the low- and high-energy spectral indices,
respectively. The
parameters were estimated by measurements of bright BATSE bursts to
be on average $\alpha\simeq-1$, $\beta\simeq-2. 25$, and $E_{0}\simeq256keV$
(Fig. \ref{fig:GRB_BandParameters}) \cite{GRB_Preece_et_al2000}. The spectral energy distribution $\nu\,F_{\nu}$
peaked at the peak energy $E_{p}\equiv(2-a)E_{0}$. Figure \ref{fig:GRB_ASpectrum} shows an example
of a spectral fit using the Band function. 
Figure \ref{fig:GRB_SyncSpectra} shows different
possible broadband synchrotron spectra from a relativistic blast wave 
that accelerates the electrons to a power-law distribution of energies, 
as believed to happen during internal shocks. 
The similarity between figures \ref{fig:GRB_ASpectrum} and \ref{fig:GRB_SyncSpectra} implies
that the prompt emission from GRBs is mostly synchrotron radiation. 

\begin{figure}[ht]
\begin{centering}
\includegraphics[width=1.9in, height=2in]{Plots/GRBs/a} \includegraphics[width=1.9in, height=2in]{Plots/GRBs/b}\includegraphics[width=1.9in, height=2in]{Plots/GRBs/eb}
\par\end{centering}

\caption{\label{fig:GRB_BandParameters} Distributions of the Band function parameters
from fits to the spectra of bright BATSE GRBs. 
\textit{Left}: Low-energy spectral index $a$, \textit{middle}: break energy $E_{0}$, \textit{right}: 
high-energy spectral index $\beta$. The units on the Y axes are number of bursts. Source: \cite{GRB_Preece_et_al2000} }
\end{figure}


\begin{figure}[ht]
\begin{centering}
\includegraphics[width=0.8\columnwidth]{Plots/GRBs/Spectrum}
\par\end{centering}

\caption{\label{fig:GRB_ASpectrum} Example of a fit to the spectrum of GRB911127 using the Band
function. Here $\alpha=-0.967\pm0.022$ and $\beta=-2.427\pm0.07$. Source: \cite{GRB_Band_et_al_1993} }

\end{figure}

\begin{figure}[ht!]
\begin{centering}
\includegraphics[width=0.8\columnwidth]{Plots/GRBs/SynchrotronSpectra.pdf}
\par\end{centering}
\caption{\label{fig:GRB_SyncSpectra}Different possible broadband synchrotron spectra from a relativistic blast wave that accelerates the electrons to a power-law distribution of energies ($N_{\gamma}\propto\gamma^{-p}$, with $\gamma$ the Lorentz factor of the electrons). The different spectra are labeled 1–5 from top to bottom. 
Different sets of physical conditions correspond to different orderings of the break frequencies: the minimal synchrotron frequency of the least energetic electron $\nu_{mu}$, the self-absorption frequency $\nu_{sa}$, and the typical synchrotron frequency of an electron whose cooling time equals the dynamical time of the system $\nu_{c}$. The similarity of these spectra to the spectrum of the prompt emission from GRBs implies that the latter is most likely synchrotron radiation. 
Source: \cite{GRB_Granot_Sari_2002}. }
\end{figure}


Ghirlanda \textit{et al}. found that the spectra of short GRBs can be better fitted by a power
law combined with an exponential cutoff at high energies \cite{GRB_Ghirlanda_et_al2004}. 
Similarly to long GRBs, they also found that the $\nu F_{\nu}$ distribution for short GRBs
peaked at an energy $E_{0}=355\pm30\,keV$.


\subsection{BeppoSAX \& HETE-2 (1996-2007)}

Because gamma rays can neither be reflected
with mirrors nor refracted with lenses, 
there are not any focusing gamma-ray telescopes
used in astronomy (see \cite{MISC_Schonfelder_2004}
for a review of the detection methods
used in gamma-ray telescopes). 
As a result, the angular resolution
of gamma-ray telescopes such as BATSE was too wide to allow
optical telescopes, which needed arcmin localizations ($(1/60)^o$), 
to search for burst counterparts. This prevented the identification
of the progenitors and the environments of GRBs, as well as the
measurement of their distances. As a result, a verification of the
cosmological origins of GRBs was still lacking. A breakthrough happened
in early 1997, when the Dutch/Italian satellite BeppoSAX \cite{URL_BEPPOSAX}
(1996-2002) detected a fading X-ray emission from long GRB970228
%(Fig. \ref{fig:GRB_BeppoSaxFirst})
. After a processing of a few
hours, a localization accurate enough for follow-up ground-based observations
at optical, radio, and other wavelengths was obtained. These observations
initially identified a fading optical counterpart, and, after
the burst had faded, long-duration deep imaging identified a very
distant ($z=0.498$) host galaxy at the location of the burst. This observation
was the first conclusive piece of evidence that long GRBs are cosmological
sources. It also paved the way for identifications of more host galaxies
and for redshift determinations through spectroscopy of the GRBs, 
and settled the distance-scale argument for long GRBs \cite{GRB_Metzger_et_al1997}. %

% \begin{figure}[ht]
% \begin{centering}
% \includegraphics[width=0.5\columnwidth]{Plots/GRBs/grb970228}
% \par\end{centering}
% 
% \caption{\label{fig:GRB_BeppoSaxFirst}BeppoSAX's observation of the afterglow
% from GRB022897 that provided the first conclusive evidence of the extragalactic
% nature of long GRBs. }
% \end{figure}

After BeppoSAX, the High-Energy Transient Explorer (HETE-2) (2000-2007)
\cite{URL_HETE2} performed more afterglow observations of high quality and helped identify
a new class of sources called ``X-Ray Flashes,'' similar to
softer GRBs identified earlier by BeppoSAX. HETE-2 also made the
first observations connecting long GRBs with Type Ic supernovae (see
subsection \ref{sub:GRB_GRB_SNCOnnection}). 

By 2005, although afterglows had been detected from about fifty long GRBs, there were
no such detections for short GRBs. The afterglows of short
GRBs were hard to detect because the detectors had to achieve precise
localizations using smaller numbers of photons, which required
more time than the case of long GRBS. By the time a precise
localization was achieved and an X-ray sensitive instrument was pointed toward the acquired location, 
the already weak afterglow of short GRBs had decayed to the point of becoming
undetectable. 

The first afterglow from a short GRB was detected by the Swift satellite, described next, 
due to its high sensitivity and fast slewing (re-pointing)
capabilities. 


\subsection{Swift (2004 - present)}

In the instruments described above, there was an $\sim8\,hr$ or longer delay
between the initial burst detection and the follow-up
observations. This resulted in the loss of important information contained
in the burst afterglow during that delay. A new satellite, called Swift \cite{URL_SWIFT}
, that could observe the afterglow of the burst swiftly after its
detection, was launched in 2004. Swift had a GRB detector combined
with a wide field X-ray and an optical/ultraviolet telescope, 
and the ability to do automated
rapid slewing. Thus, it could localize afterglows with arcsec
accuracy a minute or so after the burst at gamma-ray, X-ray, and optical
wavelengths. 

Swift's capabilities enabled us to study the transition between the
energetic and chaotic prompt emission, and the smoothly decaying softer
afterglow. These observations lead to the detection of spectral breaks
in the afterglow emission (Figs. \ref{fig:GRB_Afterglow_curves}
and \ref{fig:GRB_Afterglow_structure}), which provided support to
the collimated-emission model of GRBs and allowed us to significantly
constrain the energetics of GRBs (see subsection \ref{sub:GRB_Collimation}). 
Furthermore, it provided, for the first time, observations of the
afterglows of short $(T_{90}\lesssim2\,sec)$ bursts, which lead to redshift
measurements of short GRBs and verified the cosmological origin for
them too. 

Swift's observations of short GRBs showed that, unlike long GRBs, 
they usually originate from regions with a low star-formation rate. 
This suggested that short GRBs are related to old stellar populations, possibly
from mergers of compact-object binaries (i.e., neutron star-neutron
star or neutron star-black hole). 
Furthermore, even though supernova features such as red bumps and late-time rebrightening were detected in the afterglows
of most long GRBs close enough to allow such a detection, there were no
evidence of such features in the afterglows of long GRBs. These observations strengthened
the case for long and short GRBs having different kinds of progenitors:
compact-object binaries for short GRBs versus massive stars for long GRBs. 

\begin{figure}[ht]
\includegraphics[viewport=50bp 230bp 500bp 570bp, clip, width=1\columnwidth]{Plots/GRBs/Afterglows}
\caption{\label{fig:GRB_Afterglow_curves}Light curves of four well-sampled
GRBs exhibiting a characteristic range of potential jet break behavior. 
The light curves are composed of measurements by two of Swift's detectors:
the Burst Alert Telescope (BAT-red) and the X-Ray Telescope (XRT
- blue). Source: \cite{GRB_Kocevski_Butler2008}}
\end{figure}

\begin{figure}[ht]
\begin{centering}
\includegraphics[width=0.8\columnwidth]{Plots/GRBs/AfterglowStructure}
\par\end{centering}
\caption{\label{fig:GRB_Afterglow_structure}Synthetic sketch of a light curve
based on Swift's observations. The initial phase, denoted by ``0,'' 
corresponds to the end of the prompt emission. Four power-law light-curve
segments together with a flaring component are identified in the afterglow
phase. The components marked with solid lines are the most common, 
while the ones marked with dashed lines are observed in only a fraction
of the bursts. The typical spectral indices of the power-law decay
are shown for each segment. The break between regions III and IV occurs
simultaneously for all observed frequencies (achromatic break) and is related
to the fact that the GRB emission comes from relativistic jets. Source:
\cite{GRB_Zhang_et_al_2006}}
\end{figure}

The GRB afterglows, as observed by Swift, decayed on a power law and
progressively softened from X-rays, to optical, to radio. As of January
2008, Swift had detected 208 bursts in gamma rays, with almost all
of them having an X-ray afterglow. 

Swift is sensitive to a lower energy range ($15-150\,keV$) and to
bursts of longer durations than other detectors. 
Therefore it is more sensitive to GRBs of higher redshifts, since the signal from such GRBs is
more redshifted and time dilated. Due to its increased sensitivity to distant GRBs, 
Swift observed GRB050904, the most distant GRB ever observed. 
GRB050905 had a redshift of $z=6.295$, and when it exploded the 
age of the universe was only $\sim6\%$ of its current age. 
The redshift distribution of Swift GRBs and pre-Swift GRBs is shown in Fig. \ref{fig:GRB_Redshifts}. 
As can be seen, Swift GRBs are on average more distant than pre-Swift GRBs. 

\begin{figure}[ht]
\begin{centering}
\includegraphics[width=0.8\columnwidth]{Plots/GRBs/redshifts}
\par\end{centering}

\caption{\label{fig:GRB_Redshifts}Redshift distributions of GRBs detected
by Swift and of GRBs detected by pre-Swift satellites. The average
redshift of the Swift sample is higher than redshift of the previous observations
(2. 3 vs 1. 2), because of the greater sensitivity of Swift to distant GRBs. Source:
\cite{GRB_Gehrels_et_al2007}}
\end{figure}


%\FloatBarrier
\section{\label{sec:GRB_Hosts}The GRB Model}
According to the generally accepted model of the progenitor and the emission mechanism
of GRBs, GRBs start with a cataclysmic event, such as the merger of two
compact objects or the collapse of the core of a rotating massive
star, followed by the creation of a rapidly spinning black hole and an accreting
envelope around it (Fig. \ref{fig:GRB_Model}). This model, called the ''Collapsar model'',
was initially proposed to explain long GRBs \cite{GRB_MacFayden_Woosley1999}. However, it
was realized that the mergers of compact-object binaries that create short GRBs
also result a black hole-accretion disk system similar to the one in the collapsar model. 


\begin{figure}[ht]
\includegraphics[width=1.0\columnwidth]{Plots/GRBs/BigPlot}
\caption{\label{fig:GRB_Model}Sketch showing the process leading to the formation
of a GRB. Source: \cite{GRB_Gehrels_et_al2002}}

\end{figure}

The collapse of the accreting material that is near the equator of the envelope is somewhat
inhibited by the strong centrifugal forces. Most of the accretion
happens through two funnels that form on the poles of the black
hole (on the axis of rotation). Large amounts of energy $(\sim10^{50}\,erg/s)$
are deposited locally on the polar regions, possibly through neutrino-driven
winds \cite{GRB_Narayan_et_al1992}, magneto-hydrodynamic processes
\cite{GRB_Blandford_Znajek1977}, magnetic instabilities in the
disk \cite{GRB_Blandford_Payne_1982}. The sources for the deposited energy are
the gravitational and rotational energy of the accreting envelope
and the spinning black hole. The relative
contribution of each source (envelope or black hole) is unknown and depends on which energy-transfer
mechanism is more efficient. It is more likely that the largest fraction
is supplied by the gravitational energy of the envelope. 

Outward radiation and matter pressure gradually build up at the poles; however, they are initially
smaller than the pressure from the in-falling material. A point
is reached, at which the matter density over the poles and the accretion
rate are reduced to a large enough degree that they cannot counter-balance
the outward pressure. At that point an explosion occurs. 
A hot baryon-loaded $e^{-}, e^{+}, \gamma$ plasma (also called the
``fireball'') pushes outwards through the layers of the envelope. 
Matter and pressure gradients and magnetic fields collimate the
outflow, until it finally manages to erupt from the surface of the
object and break free in the form of two opposite narrow jets of half-opening
angle $\sim10^{o}$ (Figs. \ref{fig:GRB_JetBurst} and \ref{fig:GRB_JetBurst2}). 
Because the baryon load of the fireball plasma is small--$M_{b}c^{2}\ll E$
, where $M_{B}$ is the total mass of the baryons, and $E$ is the
total energy of the fireball--the fireball is quickly accelerated
to relativistic velocities. 

\begin{figure}[ht]
\includegraphics[width=1\columnwidth]{Plots/GRBs/jetburst}
\caption{\label{fig:GRB_JetBurst} A hyper-relativistic jet ($\Gamma\sim200$)
breaking out from the mantle of a $15M_{\odot}$ Wolf-Rayet star, 
$8\,s$ after it was launched from near the star's center. The jet's
luminosity is $3\times10^{50}\,erg/s$.  Source: \cite{GRB_Zhang_et_al_2006}}
\end{figure}
%
\begin{figure}[ht]
\includegraphics[width=0.50\columnwidth]{Plots/GRBs/SIM_SPINDISK}\includegraphics[width=0.50\columnwidth]{Plots/GRBs/SIM_JETS}
\caption{\label{fig:GRB_JetBurst2}Collapse and explosion in a 14 solar mass
Wolf-Rayet star. \emph{Left}: The iron core of a highly evolved star
collapses to a black hole. Material along the rotational axis falls
in quickly, but matter in the equatorial plane is slowed by rotation
and piles up in a disk. Here color represents log density at a time
20 seconds after the initial collapse, and the highest density in the
equatorial plane near the black hole is $9\times10^{8}\,g/cm^{3}$. 
The figure is 1800 km across, and the inner boundary is at 13 km. 
A black hole of $4. 4M_{\odot}$ has formed and has been accreting
$0.1\,M_{\odot}/s$ for the last 15 seconds. During this time, magnetohydrodynamical
processes (not included in the simulation) would launch a jet along the rotational
axis. \emph{Right}: A GRB supernova. A two-component jet was introduced
at the origin along the top and bottom axes of a star similar to the
one above. One component had $10^{51}\,erg/s$, Lorentz factor $\Gamma=50$, 
and an internal energy to mass ratio of 3. Its opening angle was about
$10^{o}$. A second component of mildly relativistic matter extended
from $30^{o}-45^{o}$ and had power $5\times10^{50}\,erg/s$ and speed
$14\times10^{3}\,km/s$. Its composition and properties reflected
those expected for a ``disk wind''
blowing off the accretion disk by viscous processes. This figure, 
$2\times10^{5}\,km$ across, shows conditions $0.94\,s$ after the jet was launched. 
Both flows are hydrodynamically focused towards the rotational axis. 
Images and caption from \cite{GRB_Zhang_et_al_2006}.}

\end{figure}


In the first stages following the ejection of the jet (preburst),
the density of the jet is very high, and any radiation produced in it is readily absorbed
instead of escaping. As a result, the jet accumulates energy, and
its bulk Lorentz factor increases further. However, as it expands, 
the optical depth is reduced, and radiation can escape from it. The
fact that the observed radiation is a power law and shows great
variability disfavors a model of a uniformly dense fireball 
expanding smoothly in the interstellar space and radiating on a thermal
spectrum. It was realized that the observed prompt emission and the 
afterglow could be produced during internal \cite{GRB_Kobayashi_et_al1997}
and external shocks \cite{GRB_Meszaros_Rees_1997}, respectively. The internal
shocks happen inside the jet and between shells of material moving
at different velocities. Such shells can be created if the 
energy-deposition mechanism is intermittent. During these shocks, 
the jet's electrons are accelerated to ultra-relativistic 
velocities and emit synchrotron radiation. 
Each peak of the prompt light curve is considered to be created during such an internal shock. 

The external shock occurs when the jet eventually collides with the ambient circumburst
medium, and smoothly and slowly decelerates. Similarly to internal shocks, relativistic electrons emit synchrotron radiation
observed as an afterglow that starts from gamma rays and gradually softens to longer wavelengths, down to radio as the jet is 
attenuated by the circumburst medium. 

While the general picture described by the collapsar model
is accepted by the scientific community, there is little consensus
regarding some of its details. The inner engine of GRBs is hidden
from us, so we can make only indirect inferences about its nature.
As a result, there is still uncertainty regarding many aspects of
the model, such as how exactly the jets are formed; which mechanism
transfers energy from the inner engine to the jets; the baryonic load
of the jets; the jets' bulk Lorentz factor; which physical processes
are involved in the internal shocks; what specific circumstances
lead to the creation of a GRB instead of just a supernova, etc. 

In the following, I will give a brief review of some of the observed
GRB properties. I will mention, where applicable, how these properties support
the collapsar model. For an extensive review on the physics of
GRBs, the collapsar model, and the progenitors and hosts of GRBs see,
\cite{GRB_Piran_2004, GRB_Meszaros_2006, GRB_Lee_Ruiz_2007, GRB_Woosley_Bloom_2006}. 


\subsection{Inner engine of GRBs}

The light curves of the prompt emission show a variability of 
milliseconds to many minutes. These short time scales imply that a compact
object is involved in the emission, with size of the order of tens
of kilometers, typical for black holes and neutron stars. The fact
that the burst duration is usually longer than the variability suggests
a prolonged and intermittent inner-engine activity in two or three
different simultaneous time scales. This disfavors any explosive model
that releases the energy at once. The total energy emitted in gamma
rays is very high, about $10^{51}\,erg$, an amount comparable to the
energy release from supernovae. The above suggest that the inner engine
of GRBs consists of a massive object, most likely a newborn black
hole, with a massive ($mass\gtrsim0.1\,M_{\odot})$ disk accreting into
it. The accretion explains the prolonged activity and the different
time scales, and the black hole satisfies the size and energy requirements. 


\subsection{Emission mechanism}

According to the collapsar model, the observed radiation is produced
at internal or external shocks. 
During these shocks, energy is transferred to the jet's electrons through a diffusive
shock acceleration mechanism \cite{GRB_Fermi_1949} in which 
magnetic field irregularities keep scattering the particles back and forth 
so they cross the same shock multiple times. During the first crossing, an electron gains an 
amount of energy of the order of $\Gamma^{2}_{sh}$, where $\Gamma_{sh}$ is the Lorentz factor
of the shock front measured in the rest frame of the jet \cite{GRB_Achterberg_et_al_2001}. 
Subsequent crossings are less efficient, and the gain is of the order of unity \cite{GRB_Achterberg_et_al_2001}. 
During these shocks, the electrons are accelerated to ultra-relativistic 
velocities ($\Gamma_{e}$ up to $\sim1000$) and emit synchrotron radiation. 
The shocks may also accelerate protons. However, the power of the synchrotron emission from protons
is considerably smaller than the power from the electrons, since an electron emits $(m_{p}/m_{e})^{2}\simeq10^{7}$ more power
through synchrotron radiation than a proton of the same Lorentz factor. Therefore the detected 
radiation is likely produced by electrons.

While the predictions of the synchrotron
model are in reasonable agreement with afterglow observations \cite{GRB_Granot_2003, GRB_Wijers_Galama1999, GRB_Panaitescu_Kumar2002}, 
there are some inconsistencies between its predictions and the observed spectral slopes \cite{GRB_Preece_et_al2002}. 
Alternative models for the emission in internal shocks include synchrotron
self-Compton \cite{GRB_Waxman_1997, GRB_Ghisellini_Celotti_1999} and
inverse Compton scattering of external light \cite{GRB_Shaviv_Dar_1995} similarly to the emission mechanism of Active Galactic Nuclei.

\subsection{Relativistic expansion}

The GRB fireball has a high radiation density, so photon pairs of center
of mass energy $\geq2\,m_{e}\,c^{2}$ should readily annihilate and create
$e^{-}e^{+}$ pairs, instead of escaping from the fireball. A calculation using
typical values yields an optical depth $\tau_{\gamma\gamma}\sim10^{15}$
\cite{GRB_Piran_1997}. In such a case, the emitted spectrum should
be thermal and should not contain an MeV or higher-energy component. 
This, in a first view creates a paradox, the ``Compactness problem,'' 
since the observed spectrum is a power law and extends up to energies of at least tens
of GeV, with no indication of a cutoff for long GRBs and up to tens of MeV for short GRBs. 

The paradox can be solved if the radiating material is moving with relativistic
velocities towards us. In such
a case, the observed GeV/MeV photons actually have a lower energy
in the fireball frame of reference. Therefore, the
optical depth of the fireball for the observed photons is actually
lower, since there is now a smaller number of photon pairs with a
center of mass energy over the annihilation threshold ($2m_{e}c^{2}$). 
If we assume that the photon energies inside the fireball are distributed
on a power law $I_{o}E^{-a}$, then this effect will decrease the
opacity by factor $\Gamma^{-2a}$, where $\Gamma$ is the bulk Lorentz factor
of the fireball \cite{GRB_Piran_2004}. Furthermore, 
because of relativistic contraction, the implied dimensions of the source
moving towards us will be smaller by a factor of $\Gamma^{2}$ than
its proper size. The power of two comes after considering the curvature of the 
emitting region (spherical-cap shape). As a result, the source's density is actually
smaller by a factor of $\Gamma^{-4}$ and the optical depth smaller
by a factor $\Gamma^{-2}$. The combined effect is
that the optical depth is actually lower by a factor of $\Gamma^{-2a-2}$
than what it would be for a non-relativistic jet, thus solving the paradox. 
Based on the above considerations and the amount of detected MeV/GeV
radiation from GRBs, lower limits on the bulk Lorentz factor of $\Gamma\gtrsim15$
were placed for short GRBs \cite{GRB_Nakar_2007} and
$\Gamma\gtrsim100$ for long GRBs \cite{GRB_Lithwick_Sari_2001}. 

Another piece of evidence supporting the case for relativistic motion
of the ejecta comes from the fact that estimates of the size of the
afterglow two weeks after the burst, independently provided by
radio scintillation \cite{GRB_Goodman_1997} and lower-frequency self
absorption \cite{GRB_Katz_Piran_1997}, can be explained only by assuming
relativistic expansion. 

%\FloatBarrier
\subsection{\label{sub:GRB_Collimation}Energetics and collimated emission}

The afterglow light curves of GRBs exhibit achromatic spectral breaks (Fig. \ref{fig:GRB_Afterglow_structure}) that
can be explained by assuming that the geometry of the ejecta
is conical (on two opposite jets) instead of spherical. Figure \ref{fig:GRB_Beams}
shows how this can happen. Because the fireball is moving with relativistic
velocities, its emission is beamed. Consider an observer that is inside
the projection of the emission cone of the fireball. Initially, when the bulk
Lorentz factor of the fireball is very high, the relativistically-beamed
radiation will be emitted in a very narrow cone. As a result, the
observer will not be able to see the emission from a part of the fireball.
Such a case is shown in the top picture of figure \ref{fig:GRB_Beams}, 
in which radiation from the sides of the fireball is clearly not visible
by the observer. As the GRB progresses, the surface of the fireball
expands (as $\propto t^{2}$), and the emitted radiation density drops
with the same rate, causing a gradual decrease in the observed brightness
of the burst. However, because of the expansion, the bulk Lorentz
factor is reduced, and the relativistic beaming becomes wider. As a
result, a larger fraction of the surface of the fireball will come
in the field of view of the observer (middle picture), reducing the
decay rate of the observed GRB brightness (now $\sim\propto t^{-1. 2}$
instead of $\sim\propto t^{-2}$). Eventually, all of the surface
of the burst becomes visible to the observer, and a gradually
increasing fraction of the fireball is no longer able to be seen.
The decay rate of the burst's brightness now depends only on the expansion
of the fireball's surface and becomes proportional to $t^{-2}$. This
transition, appearing as an achromatic break on the afterglow light curve, 
has been observed on many GRBs. For the GRB afterglows with no observed jet
breaks, it is assumed that the breaks happened at a time long after
the bursts, when no observation data exist. %
\begin{figure}[ht]
\begin{centering}
\includegraphics[height=0.8\textheight]{Plots/GRBs/Beams}
\par\end{centering}

\caption{\label{fig:GRB_Beams}Sketch showing how the relativistic beaming combined
with  collimated matter emission produces an achromatic spectral break
in the afterglow curve of GRBs. Source: \cite{GRB_Gehrels_et_al2002}}
\end{figure}


The typical GRB gamma-ray fluences at the earth are of the order of $10^{-5}\,erg/cm^{2}$. 
If we assumed an isotropic emission from GRBs, then this fluence, combined with 
the distance scale of GRBs (say $z=2$), would result to an isotropically-emitted energy
of $E_{iso}\simeq10^{53}\,erg$. Such an energy emission is considerably
higher than the emission from a typical supernova ($10^{51}\,erg$
in few months or $10^{49}\,erg$ in hundreds of seconds), and is difficult
to explain. However, the fact that the emission geometry is conical
ameliorates these energy requirements. 
If the emission actually happened in a solid angle $\Delta\Omega$, 
then the true amount of emitted energy is 
\begin{eqnarray*}
E_{true} & = & 2\,E_{iso}\,\Delta\Omega/4\pi\\
 & = & 2\,E_{iso}\,\frac{1-cos(\theta_{jet})}{2}\\
 & \simeq & E_{iso}\,\frac{\theta_{jet}^{2}}{2},\end{eqnarray*}
where $\theta_{jet}$ is the half opening angle of the emission cone. 
Frail \textit{et al.} \cite{GRB_Beaming_Frail2001} estimated $\theta_{jet}$
for a sample of GRBs, based on the occurrence time of the achromatic break in
their afterglow curves. Based on $\theta_{jet}$, they calculated the true amount of emitted
energy from the isotropic-equivalent amount. Their result (Fig. \ref{fig:GRB_CorrectedEnergy})
showed that even though the isotropic-equivalent emitted energy spans a wide energy range
$(4\times10^{52}-2\times10^{54}\,erg)$, the true amount of emitted energy spans a considerably
narrower energy range centered at $\sim3\times10^{50}\,erg$. This shows that the energy emission
of GRBs is comparable to that of supernovae, and suggests that GRBs have a standard energy reservoir.
The fact that the emission is conical also increases
the implied rate of GRBs by the same factor ($\simeq\theta_{jet}^{2}$), since only GRBs with their
emission cones pointing to the earth are detected. 

\begin{figure}[ht]
\begin{centering}
\includegraphics[width=0.8\columnwidth]{Plots/GRBs/BeamingEnergy}
\par\end{centering}

\caption{\label{fig:GRB_CorrectedEnergy}GRB energetics:
distribution of the isotropic-equivalent
emitted energy for a selection of GRBs with known redshifts \textit{(top)}, 
distribution of the geometry-corrected emitted energy for the same
GRBs \textit{(bottom)}. Arrows are plotted for five GRBs to indicate lower or upper
limits to the geometry-corrected energy. Source: \cite{GRB_Zhang_et_al_2006}}
\end{figure}



\subsection{Progenitors of GRBs}

There are multiple observational pieces of evidence that suggest that
not all GRBs are the same, and that there are different kinds of
progenitors and inner engines. Specifically, the duration and the hardness ratio-duration
distributions (Figs. \ref{fig:GRB_T90} and \ref{fig:GRB_HardnessRatio}) 
show that there are two kinds of bursts: short-hard
bursts and long bursts. Deep long-duration observations of the
optical afterglows of short bursts did not show any evidence of an
associated supernova \cite{GRB_Bloom_et_al2006, GRB_Hjorth_et_al2005, GRB_Fox_et_al2005}.
On the other hand, supernova-emission spectra were detected superimposed on the afterglows of most of the long
GRBs ($\sim20$ GRBs) that were close enough ($z\lesssim1$) to allow for such a detection \cite{GRB_Soderberg_et_al2006}. 

Short duration bursts are primarily observed in regions with low or
no star formation, therefore they are likely to be related to old stellar
populations. This suggests that these bursts could be the result of mergers
of compact binaries, such as neutron star-neutron star or neutron
star-black hole. The binary loses rotational energy through the
emission of gravitational radiation and eventually merges, forming
a black hole and an accretion disk surrounding it. The resulting system, 
then, produces a GRB in a way similar to
the collapsar model described above. 

Long bursts are observed in regions with high star formation and are
usually accompanied by supernovae, implying that they are related
to the death of massive stars (see subsection \ref{sub:GRB_GRB_SNCOnnection} for more details on
the GRB-supernova connection). The massive star involved is most likely
a Wolf-Rayet star,
\footnote{Massive stars ($Mass>20\,M_{\odot}$) that rapidly lose their outer envelope by
means of a very strong stellar wind.}
given that absorption features in the afterglow of long
GRBs \cite{GRB_Moeller_et_al2002} were explained by the presence
of the fast-moving wind of such a star. Furthermore, the fact that 
long-GRB counterparts are located within the blue parts of galaxies argues
against high-velocity progenitors (such as merging neutron stars). 
The above suggest that long GRBs likely come from the collapse of
the core of a Wolf-Rayet star that for some reason created a GRB instead
of just a supernova. Some of the differences between short and long GRBs come from the fact that
the engine of long GRBs operates at the center of a collapsing star, 
therefore it is covered by the mantle of the star, while the engine
of short GRBs is more or less exposed. 


\subsubsection{\label{sub:GRB_GRB_SNCOnnection}Long GRB-supernova connection}

In 1998, the optical telescope ROTSE discovered a transient emission 
coincident in space and time with BeppoSAX/BATSE long GRB980425 \cite{GRB_ROTSE_980425}. 
The location, spectrum and light curve of the optical transient lead
to its identification as a very luminous Type Ic supernova%
\footnote{A Type Ic supernova has no hydrogen in its spectrum and lacks strong
lines of HE I and Si II. } (SN 1998bw) \cite{GRB_Galama_et_al1998, GRB_Kulkarni_et_al1998}. This
detection was a first of its kind, and suggested that long GRBs are
related to supernovae, and therefore to the deaths of massive stars. 
Because GRB980425 was very subenergetic comparing to other GRBs (isotropic
energy emitted was $\sim8\times10^{47}\,erg$ instead of the usual
$10^{51}-10^{54}\,erg$), the supernova-GRB connection was initially called into question. 
However, a few years later, a similar event happened. Emission from
a supernova (SN2003dh \cite{GRB_Hjorth2003}) was detected on the
afterglow of long GRB030329. This time, the associated GRB
had a normal energy. In addition to those events, there have also been red
emission ``bumps'' superimposed on the afterglows of GRBs, with
color, timing, and brightness consistent with the emission of a Type
Ic supernova similar to SN 1998bw (see \cite{GRB_Woosley_Bloom_2006}
and references therein). 

Based on the above, it is now believed that most, if not all, long
GRBs are accompanied with a Type Ic supernova. It should be noted, 
however, that not all Type Ic supernova create a GRB. The specific
conditions that lead to the creation of a GRB is one of the open questions
of the field. Observational and theoretical evidence imply that high
rotational speeds, high progenitor masses, and regions of low
metallicity \cite{GRB_Fynbo_etal2003, GRB_MacFayden_Woosley1999} favor
the creation of GRBs. 

The collapsar model of GRBs can accommodate the existence of a Type Ic supernova. 
Specifically, the GRB and the underlying supernova are powered
by different sources. The supernova and the $^{56}Ni$ that makes
it bright are produced by a sub-relativistic disk wind \cite{GRB_MacFayden_Woosley1999}. 
The wind begins as protons and neutrons, in about equal proportions, 
and after it cools, it ends up as $^{56}Ni$. The nickel comes out
in a large cone surrounding the GRB jet. 


